Life on Exoplanets In the Habitable Zone of M-Dwarfs?

Exoplanets orbiting in the habitable zone around M-dwarf stars have been prime targets in the search for life due to the long lifetimes of the host star, the prominence of such stars in the galaxy, and the apparent excess of terrestrial planets found around M-dwarfs. However, the heightened stellar activity of M-dwarfs and the often tidally locked planets in these systems have raised questions about the habitability of these planets. In this letter we examine another significant challenge that may exist: these systems seem to lack the architecture necessary to deliver asteroids to the habitable terrestrial planets, and asteroid impacts may play a crucial role in the origin of life. The most widely accepted mechanism for producing a stable asteroid belt and the late stage delivery of asteroids after gas disk dissipation requires a giant planet exterior to the snow line radius. We show that none of the observed systems with planets in the habitable zone of their star also contain a giant planet and therefore are unlikely to have stable asteroid belts. We consider the locations of observed giant planets relative to the snow line radius as a function of stellar mass and find that there is a population of giant planets outside of the snow line radius around M-dwarfs. Therefore, asteroid belt formation around M-dwarfs is generally possible. However, we find that multi-planetary system architectures around M-dwarfs can be quite different from those around more massive stars.

==> response.tex <==
We thank the referee very much for the timely report and the useful comments that have improved the manuscript. We have re-queried the exoplanet data since our first draft and relax the filters so that we may include more systems in our analysis.  We no longer limit our analysis to single star systems or only the systems that the exoplanet archive reports a default stellar mass for.  We use only default values for planet parameters but not necessarily for stellar parameters, which leads to more systems in our analysis. We have addressed all of the points raised and we outline our response to each below. 

Reviewer's Comments:
In this paper, the authors address the interesting question of whether bombardment of planets in the habitable zone of M-dwarfs could be necessary for the development of life. The issue of cometary/asteroidal bombardment is one of great interest recently, and the authors focus on the positive aspects of asteroidal impacts, operating under the hypothesis that the delivery of asteroids to potentially habitable planets is "crucial... in the origin of life". The authors then assume that a Jupiter-analog is necessary for the development of an asteroid belt, which is subsequently necessary for the delivery of asteroids to the habitable planet's orbit (lines 180-185). Under the assumption that a Jupiter-analog is necessary to create an asteroid-belt-analog, which is needed for the development of life on habitable planets, the authors look at the observational data and compare the locations of Jovian-type planets to the ice lines in observed exoplanet systems around M-type stars (as well as a sample of F-, G- and K-type stars, for comparison) and state that the conclusion is that since planets around M-dwarfs do not have Jovians exterior to the ice line, then they do not have stable asteroid belts. 

The authors have written a creative paper, unifying multiple aspects of exoplanet occurrence, system architecture, and habitability. The idea put forward by the paper is interesting and merits publication. However, I have some comments that the authors should consider before the paper is suitable for publication. 

Major Comments: 

1. The authors summarize their logic quite nicely in their conclusion. My major concern is that the statements in that summary have not been appropriately justified (either with citations to the literature, or with new work as needed). As stated in the conclusion: "Giant planets exterior to the snow line radius are necessary for preventing planet formation there, creating an asteroid belt, and the delivery of the volatile rich asteroids to the inner terrestrial system after gas disk dispersal." - this is not sufficiently justified in the paper, as the statement "necessary" means that no other mechanism can deliver these asteroids. If the claim is, as indicated on line 166, that you really need a specific asteroid-belt-analog with the same dynamical properties in order to deliver asteroids to a habitable planet - then this raises a second major point. How do we know that only the particular combinations of orbital properties and secular resonances present in the asteroid belt can deliver asteroids inwards? The authors have given citations on lines 169 - 175 that show our own asteroid belt can do it, but have not sufficiently justified that another geometry of planetesimal debris and planetary architecture could NOT provide the same effect, particularly at early times before the debris disk dissipates. The Petit and Martin references are a good start, but has anyone shown that you cannot deliver asteroids (or comets, etc) without a Jupiter? Can the authors provide either some citations or numerical simulations suggesting that this is true (or, alternatively, de-scope the conclusion to reflect these limitations)? 

RESPONSE:
In the absence of any giant planets, there are no resonances and so there will be no instability (eccentricity growth) in a belt to deliver a significant amount of asteroids to the inner disk regions. Other effects that may drive asteroids in include asteroid-asteroid interactions or the Yarkovsky effect, but these mechanisms operate on longer timescales and are unlikely to provide a late-stage bombardment similar to what the early Earth experienced.  We expand on the point in lines 203-215.

2. Observational bias - can the authors comment on how "complete" the systems they consider are? Have Jovians been ruled out with RVs in any of these systems, or is it possible they are there and we just haven't observed them? You do mention that some of the detections come from microlensing, which is very biasing, but how sure are we that what we see isn't just a consequence of the ways in which these systems have been observed.

RESPONSE:  It is possible the systems do have long period giant planets that observations are biased against.  However, we are mainly interested in giant planets not too far from the snow line so that an asteroid belt may form just interior to the snow line.  RV observations are more sensitive to low mass stars and giant planets that are not too far from the snow line would likely raise TTVs on the inner smaller planets.  For these reasons, while the observations may be missing long period giant planets, the lack of giant planets around low mass stars, not too far from the snow line, is likely real.  We clarify this in lines 156-186.


Minor Comments:

A. There are many places where statements are inadequately cited. For example, the sentences ending on lines: 50, 53, 61, 67, 93, 199. A good example of citation usage is given ending on line 71. I urge the authors to consider where (in addition the places I noted) claims are not common sense or general knowledge, and provide citations as necessary. For example, the lines 57-61 discuss the "considerable skepticism" on a hypothesis, but do not provide where this criticism might be found. 

RESPONSE: Citations have been added at the recommended locations and elsewhere as they were needed.

B. Line 118 - I think that all 43 of the 43 systems should have radius and semi-major axis (which is determined directly from orbital period and stellar mass). Does this statement mean that the HEC does not report semi-major axis, but it can be easily calculated? The authors should be able to get these values from the IPAC catalog, or calculate themselves, and then figure 1 could have a lot more rows. 

RESPONSE:  We have extended our analysis to multi-star systems instead of limiting it to only single star systems as we had previously, bringing the total number of systems that contain at least one habitable planet to 48. We now also include an additional plot for the systems that have mass measurements since not all systems have mass measurements or radius measurements for all the planets in a system.  The two plots in Figure 1 now show all of the multi-planet systems that contain at least one planet in the habitable zone.  We do not show single planet systems since the lack of an exterior giant planet companion is given.  Yes, the HEC reports only orbital periods for the habitable planets.


C. There are a few locations throughout the draft where details are unclear, which may be due to typos. I will list them here. 
I. Line 114 - "less massive than 1 M_sun" - typo? Since one point in Figure 1 has a stellar mass above this value?

RESPONSE:  We have updated the text to read "M,K, and G-type Stars".

Ii. Lines 142 - "Kepler detection limit" is a bit vague - planets have been found with Kepler with orbital periods of greater than 200 days. 

RESPONSE:  We have clarified that while most planets require three transit observations before they can be confirmed, which limits the orbits that may be observed, two transits with high signal-to-noise ratios are sufficient which allows longer period planets to be found (lines 169-176)

Iii. Lines 146 - 150: TTV signal does not increase with orbital period as stated - it decreases non-monotonically with period ratio (with spikes in TTV amplitude near MMRs). As written, this sentence is not true. 

RESPONSE:  We have removed this sentence but mention giant planets not too far from the ice line would likely raise TTVs on the inner planetary system.

Iv. Line 292 - what equation are you using? I am confused because you should not need to assume e=0 to get the semi-major axis from the orbital period. 

RESPONSE: We clarify that we use Kepler's third law to estimate the semi-major axis for planets with only orbital period measurements and add the Equation as Eq. 1.


D. I think Figure 1 was very clear and well-made. 

RESPONSE:  Thank you! We have updated it to include all multi-planet systems with a habitable planet and with data queried on the dates listed in Footnotes 1 and 2.

E. On line 155, the authors state they used the values from IPAC's exoplanet archive. I suggest they put in a date at which the data was pulled, so that the plot can be recreated later (the data there is constantly being updated). 

RESPONSE:  We have added the dates in Footnotes 1 and 2.

F. Similarly, in Figure 2, I was not convinced by the top panel, but the bottom panel was very useful and illustrated the conclusion clearly. 

RESPONSE:  We have updated this plot to reflect the data queried on the date listed.


G. For Figure 3, it might be helpful to say what the asterisk means in the caption. Also, when you say resonance systems might form differently - I wonder how this relates to the "you need a Jovian to make an asteroid belt issue". Is resonant formation different enough that that may not hold? Izidoro suggests that collisions might be a lot more common.

RESPONSE:  We have updated the caption for Figure 3.  We have also updated Figure 3 to include data queried on the listed date and to also include systems with more than one star.  While we use default parameters for the planets we now relax this constraint for stellar mass so we may include more systems.  With the new data it's not apparent that planets around low mass stars do form closer together and are more likely to form in resonant chains than around higher mass stars and so we have removed this point from the text.  We have added the Izidoro citation to line 259.

Data editor's review:
One of our data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.

The authors indicated that they used IPAC data or products in their article. The next step is to identify the DOI for the archival data: 

https://www.ipac.caltech.edu/dois 

and then cite this DOI in the revised manuscript. Citation instructions are available at the AAS Journals' Author Instructions. 

https://journals.aas.org/aastexguide/#softwareandthirdparty 

The authors can use https://www.doi2bib.org to generate the necessary bibtex.

RESPONSE: A citation for the data has been added.
